Generalisation of DGLAP equations to massive partons

DGLAP evolution equations are modified in order to use all the quark families in the full scale range, satisfying kinematical constraints and sumrules, thus having complete continuity for the pdfs and observables. Some consequences of this new approach are shown.

==> coef.tex <==
\subsubsection {Coefficient functions Solution I}
The scheme changes needed to obtain the three structures function $a=L,2,3$
are:
 \begin{eqnarray}
 ^a g (Q^2)&=&
-\phi \otimes\tilde{\rc^a}_{qg} 
\otimes  g (Q^2)
-\bigl( \rc^a_{NS}+\phi \otimes \tilde{\rc^a_S}\bigr)
\otimes  \Sigma (Q^2)\\
   ^a  \Sigma (Q^2)&=&
\phi \otimes\tilde{\rc^a}_{qg} \otimes  g (Q^2)
+  \bigl( \rc^a_{NS}+\phi \otimes \tilde{\rc^a_S} \bigr) \otimes \Sigma (Q^2)\\
  ^a  l_{LN} (Q^2)&=&
                                 \rc^a_{NS} \otimes  l_{LN} (Q^2)\\
   ^a h  (Q^2)&=&
 \phi_h \otimes\tilde{\rc^a}_{qg} \otimes  g (Q^2)
+                                 \rc^a_{NS} \otimes  h (Q^2)
+\phi_h \otimes \tilde{\rc^a_S}  \otimes \Sigma (Q^2)
\end{eqnarray}

Notice that the total momentum x distribution is invarient under those 
scheme changes.

